New Physics at the LHC: A Les Houches Report. Physics at Tev Colliders 2007 -- New Physics Working Group

We present a collection of signatures for physics beyond the standard model that need to be explored at the LHC. The signatures are organized according to the experimental objects that appear in the final state, and in particular the number of high pT leptons. Our report, which includes brief experimental and theoretical reviews as well as original results, summarizes the activities of the "New Physics'' working group for the "Physics at TeV Colliders" workshop (Les Houches, France, 11-29 June, 2007).

==> commands.tex <==
% Main file
%

\makeatletter
\def\myaddcontentsline@toc#1#2#3{%
   \addtocontents{#1}{\protect\thispagestyle{empty}}%
   \addtocontents{#1}{\protect \vspace{-1cm}}
   \addtocontents{#1}{\protect\contentsline{#2}{#3}{}}
   \addtocontents{#1}{\protect \vspace{-.8cm}}}
\def\myaddcontentsline#1#2#3{%
  \expandafter\@ifundefined{addcontentsline@#1}%
  {\addtocontents{#1}{\protect \vspace{-1cm}}
  \addtocontents{#1}{\protect\contentsline{#2}{#3}{}}
  \addtocontents{#1}{\protect \vspace{-.8cm}}}
  {\csname addcontentsline@#1\endcsname{#1}{#2}{#3}}}
\makeatother

\makeatletter
\def\mysuperaddcontentsline@toc#1#2#3{%
   \addtocontents{#1}{\protect\thispagestyle{empty}}%
   \addtocontents{#1}{\protect \vspace{.6cm}}
   \addtocontents{#1}{\protect\contentsline{#2}{#3}{\thepage}}
   \addtocontents{#1}{\protect \vspace{-.5cm}}}
\def\mysuperaddcontentsline#1#2#3{%
  \expandafter\@ifundefined{addcontentsline@#1}%
  {\addtocontents{#1}{\protect \vspace{.6cm}}
  \addtocontents{#1}{\protect\contentsline{#2}{#3}{\thepage}}
  \addtocontents{#1}{\protect \vspace{-.5cm}}}
  {\csname addcontentsline@#1\endcsname{#1}{#2}{#3}}}
\makeatother

\newcommand{\superpart}[1]{\clearpage \thispagestyle{empty}  \vphantom{blabla}\vspace{5cm} \centerline{\huge #1} 
\mysuperaddcontentsline{toc}{part}{\protect\numberline{} \hspace{-2cm}#1}%
\clearpage}
   
\newcommand{\AddToContent}[1]{\myaddcontentsline{toc}{part}{\protect  \textit{\hspace{1.5cm} \small#1}}}

\renewcommand{\thepart}{\arabic{part}}
\renewcommand{\thesubsubsection}{\arabic{section}.\arabic{subsection}.\arabic{subsubsection}}


%


% Paraphoton by E. Boos et al.
%
\newcommand{\paraphotonlsim}{\stackrel{<}{_\sim}}
%\newcommand{\gsim}{\stackrel{>}{_\sim}}
%\newcommand{\met}{\mbox{\ensuremath{\slash\kern-.7emE_{T}}}}
%\newcommand{\mpt}{\mbox{\ensuremath{\slash\kern-.7emp_{T}}}}
\newcommand{\paraphotonme}{\mbox{\ensuremath{\slash\kern-.7emE}}}
%\newcommand{\missp}{\mbox{\ensuremath{\slash\kern-.7emp}}}
%

% LSTC by K. Lane et al.  
\newcommand\LSTCtpi{\pi_T}
\newcommand\LSTCifb{{\rm fb}^{-1}}
\newcommand\LSTCta{a_T}
\newcommand\LSTCtropm{\rho_{T}^\pm}
\newcommand\LSTCra{\rightarrow}
\newcommand\LSTCtro{\rho_{T}}
\newcommand\LSTCgev{{\rm GeV}}
\newcommand\LSTCellp{\ell^+}
\newcommand\LSTCellm{\ell^-}
\newcommand\LSTCellpm{\ell^\pm}
\newcommand\LSTCtpipm{\pi_T^\pm}
\newcommand\LSTCtev{{\rm TeV}}
\newcommand\LSTCLtc{\Lambda_{TC}}
\newcommand\LSTCsimle{\mathrel{
   \rlap{\raise 0.511ex \hbox{$<$}}{\lower 0.511ex \hbox{$\sim$}}}}
\newcommand\LSTCsimge{\mathrel{%
   \rlap{\raise 0.511ex \hbox{$>$}}{\lower 0.511ex \hbox{$\sim$}}}}
\newcommand\LSTCtom{\omega_{T}}
\newcommand\LSTCbe{\begin{equation}}
\newcommand\LSTCee{\end{equation}}
\newcommand\LSTCtpip{\pi_T^+}
\newcommand\LSTCtpiz{\pi_T^0}
\newcommand\LSTCtpimp{\pi_T^\mp}
\newcommand\LSTCts{\thinspace}
\newcommand{\LSTCthw}{\ensuremath{\theta_W}}
\newcommand\LSTCbea{\begin{eqnarray}}
\newcommand\LSTCeea{\end{eqnarray}}
\newcommand\LSTCtroz{\rho_{T}^0}
\newcommand\LSTCtrho{\rho_T}
\newcommand\LSTCtpipr{\pi_T^{0 \prime}}
\newcommand\LSTCpb{{\rm pb}}
\newcommand\LSTCjet{{\rm jet}}
\newcommand\LSTCetmiss{\LSTCslashchar{E}_T}
\newcommand{\LSTCslashchar}[1]%
        {\kern .25em\raise.18ex\hbox{$/$}\kern-.75em #1}
\newcommand\LSTCCL{{\cal L}}
%\newcommand\LSTCCCL{$\CL$}
\newcommand\LSTCat{a_T}
\newcommand\LSTCfb{{\rm fb}}
\newcommand\LSTCCO{{\cal O}}
%\newcommand\CCO{$\CO$}

% interface by P. Skands et al.
\newcommand{\interfacettt}[1]{\texttt{#1}}
\newcommand{\interfacetsc}[1]{\textsc{#1}}
\newcommand{\interfacecode}[1]
 {\hspace*{0.075\textwidth}\begin{minipage}{0.9\textwidth}{\small\interfacettt{#1}}
\end{minipage}\newline}

% walker by D. Walker
%\def\s{\rm s}
\def\walkerttb{t\bar t}
\def\walkeretmiss{E\!\!\!\!\slash_{T}}
%

% KKgluon by G. Moreau et al.
\newcommand{\KKgluonlsim}{\raisebox{-0.13cm}{~\shortstack{$<$ \\[-0.07cm] $\sim$}}~}  
\newcommand{\KKgluongsim}{\raisebox{-0.13cm}{~\shortstack{$>$ \\[-0.07cm] $\sim$}}~}  
\newcommand{\KKgluonmkk}{M_{\rm KK}}  
\newcommand{\KKgluonvkk}{V_{\rm KK}}  





% toppartners by Boos et al.
\newcommand{\BCNSeps}{\varepsilon}
%

% WW scattering by R. Rosenfeld et al.
\def\WWgsim{~\rlap{$>$}{\lower 1.0ex\hbox{$\sim$}}\;}


